HLSDataset: Open-Source Dataset for ML-Assisted FPGA Design using High Level Synthesis

Machine Learning (ML) has been widely adopted in design exploration using high level synthesis (HLS) to give a better and faster performance, and resource and power estimation at very early stages for FPGA-based design. To perform prediction accurately, high-quality and large-volume datasets are required for training ML models.This paper presents a dataset for ML-assisted FPGA design using HLS, called HLSDataset. The dataset is generated from widely used HLS C benchmarks including Polybench, Machsuite, CHStone and Rossetta. The Verilog samples are generated with a variety of directives including loop unroll, loop pipeline and array partition to make sure optimized and realistic designs are covered. The total number of generated Verilog samples is nearly 9,000 per FPGA type. To demonstrate the effectiveness of our dataset, we undertake case studies to perform power estimation and resource usage estimation with ML models trained with our dataset. All the codes and dataset are public at the github repo.We believe that HLSDataset can save valuable time for researchers by avoiding the tedious process of running tools, scripting and parsing files to generate the dataset, and enable them to spend more time where it counts, that is, in training ML models.

==> 8_discussion.tex <==
\section{Discussion and Future Work} \label{discussion}


\RL{In this paper, we have demonstrated the efficacy of HLSDataset through two ML case studies. To achieve higher accuracy, a more balanced training dataset is desired~\cite{batista2004study} for ML training. By characterizing and identifying similarities between each data point in HLSDataset~\cite{panda2018wait}, a more balanced and representative HLSDataset subset can be obtained and used in ML training scenarios. }

\RL{HLSDataset focused on single-bit-stream scenarios. In FPGA-based datacenters, one requested job can consist of multiple stages, which requires using dynamic reconfiguration on a single board or deploying on multi-board clusters.
A multi-stage HLSDataset can be generated by using recurrent neural networks to model the time sequence of each stage (single data point)~\cite{bergsma2021generating}. }

%Now I think we don't need to include this. It feels very defensive.
%I copied this from the FCCM rebuttal
%Our dataset is currently generated using the 2022.2 version of Xilinx Vivado. The dataset will still be useful even when a new version of tool comes out. Firstly, dataset construction flow and infrastructure will also be opened to public, the dataset can be extended/updated for new benchmarks, new FPGA type, new version of tools. This flow already works for multiple versions of Xilinx Vivado, and we believe limited efforts are needed for other versions of tools. Secondly, our dataset can still be useful even if it becomes old compared to the versions of tools. Our dataset is useful for the academic study of ML model in HLS domain where new ML techniques, ML to solve new problems can be easily conducted with our dataset. The dataset will also have acceptable lifetime if tool algorithms do not have huge changes. In summary, we think our dataset can sufficiently help the ML study in HLS domain of FPGA community.


